Waffling around for Performance: Visual Classification with Random Words and Broad Concepts

The visual classification performance of vision-language models such as CLIP has been shown to benefit from additional semantic knowledge from large language models (LLMs) such as GPT-3. In particular, averaging over LLM-generated class descriptors, e.g. "waffle, which has a round shape", can notably improve generalization performance. In this work, we critically study this behavior and propose WaffleCLIP, a framework for zero-shot visual classification which simply replaces LLM-generated descriptors with random character and word descriptors. Without querying external models, we achieve comparable performance gains on a large number of visual classification tasks. This allows WaffleCLIP to both serve as a low-cost alternative, as well as a sanity check for any future LLM-based vision-language model extensions. We conduct an extensive experimental study on the impact and shortcomings of additional semantics introduced with LLM-generated descriptors, and showcase how - if available - semantic context is better leveraged by querying LLMs for high-level concepts, which we show can be done to jointly resolve potential class name ambiguities. Code is available here: https://github.com/ExplainableML/WaffleCLIP.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -pdf \"$_[0]\"" );
    }
}

==> tables/additional_benchmarks_sup.tex <==
\begin{table}[t]
\centering\resizebox{0.48\textwidth}{!}{
\begin{tabular}{l|lll|l}
\toprule
\textbf{ViT-B/32} & Flowers102 & FGVCAircraft & Stanford Cars & \textbf{Avg} \\
\hline
CLIP & 62.89 & 24.99 & 58.54 & 48.81\\
DCLIP \cite{dclip} & 64.01 & 26.94 & 57.08 & 49.34\\

\hline
\texttt{Waffle}CLIP & 66.27 \small$\pm0.26$ & 25.66 \small$\pm0.19$ & 58.91 \small$\pm0.17$ & 50.28 \small$\pm0.21$\\
+ Concepts & \textbf{67.19} \small$\pm0.19$ & 28.44 \small$\pm0.22$ & \textbf{59.70} \small$\pm0.12$ & \blue{\textbf{51.78}} \small$\pm0.18$\\
+ GPT dsc. + Conc. & 66.71 \small$\pm0.39$ & \textbf{28.96} \small$\pm0.37$ & 59.33 \small$\pm0.14$ & 51.67 \small$\pm0.32$\\
\bottomrule
\end{tabular}
}
\centering\resizebox{0.48\textwidth}{!}{
\begin{tabular}{l|lll|l}
\toprule
\textbf{ViT-L/14} & Flowers102 & FGVCAircraft & Stanford Cars & \textbf{Avg} \\
\hline
CLIP & 74.73 & 44.88 & 76.42 & 65.34\\
DCLIP \cite{dclip} & 78.16 & \textbf{51.04} & 75.13 & 68.11\\
\hline
\texttt{Waffle}CLIP & 76.17 \small$\pm0.27$ & 48.72 \small$\pm0.40$ & \textbf{76.71} \small$\pm0.12$ & 67.20 \small$\pm0.29$\\
+ Concepts & 78.12 \small$\pm0.18$ & 49.45 \small$\pm0.26$ & 76.41 \small$\pm0.08$ & 67.99 \small$\pm0.19$\\
+ GPT dsc. + Conc. & \textbf{78.57} \small$\pm0.22$ & 50.79 \small$\pm0.47$ & 76.23 \small$\pm0.14$ & \blue{\textbf{68.53}} \small$\pm0.31$\\
\bottomrule
\end{tabular}
}
\centering\resizebox{0.48\textwidth}{!}{
\begin{tabular}{l|lll|l}
\toprule
\textbf{ResNet50} & Flowers102 & FGVCAircraft & Stanford Cars & \textbf{Avg} \\
\hline
CLIP & 61.36 & 21.15 & 54.05 & 45.52\\
DCLIP \cite{dclip} & 64.86 & 24.48 & 52.59 & 47.31\\
\hline
\texttt{Waffle}CLIP & 65.25 \small$\pm0.34$ & 23.66 \small$\pm0.04$ & 53.77 \small$\pm0.23$ & 47.56 \small$\pm0.24$\\
+ Concepts & 66.58 \small$\pm0.20$ & 24.25 \small$\pm0.09$ & \textbf{54.11} \small$\pm0.23$ & 48.31 \small$\pm0.18$\\
+ GPT dsc. + Conc. & \textbf{67.11} \small$\pm0.24$ & 24.80 \small$\pm0.32$ & 53.64 \small$\pm0.12$ & \blue{\textbf{48.52}} \small$\pm0.24$\\
\bottomrule
\end{tabular}
}
\caption{We find consistent performance improvements with \ourmodel, and when utilizing additional high-level concept guidance in three additional benchmarks. Some benchmarks may not benefit from additional descriptors (see \textit{Stanford Cars}), but high-level concepts or \texttt{Waffle}CLIP still prove useful.}
\label{sup:tab:additional_benchmarks}
\end{table}

==> tables/concepts.tex <==
\begin{table}[t]
\centering\resizebox{0.24\textwidth}{!}{
\begin{tabular}{l|l|l}
\toprule
Method & Concept & Usable \\
\hline
ImageNet (V2) & \texttt{Object} & No \\
ImageNet & \texttt{Object} & No \\
CUB200  & \texttt{Bird} & Yes \\
EuroSAT  & \texttt{Land Use} & Yes \\
\bottomrule
\end{tabular}
}
\centering\resizebox{0.23\textwidth}{!}{
\begin{tabular}{l|l|l}
\toprule
Method & Concept & Usable \\
\hline
Places365  & \texttt{Place} & Yes \\
Food101  & \texttt{Food} & Yes \\
OxfordPets  & \texttt{Breed} & Yes \\
DTD  & \texttt{Adjective} & No \\
\bottomrule
\end{tabular}
}
\caption{GPT-3 generated high-level concepts for each dataset, and their usability as prompt extensions.}
\label{tab:concepts}
\end{table}

==> tables/correct_prompt.tex <==
% \begin{table}[t]
% \centering\resizebox{0.48\textwidth}{!}{
% \begin{tabular}{l|llll}
% \toprule
% Method & ImageNet & ImageNetV2 & CUB200 & EuroSAT \\
% \hline
% CLIP w/o  & 51.87 & 58.47 & 51.98 & 45.48 \\
% CLIP + P  & 54.61 & 62.06 & 51.92 & 37.71 \\
% \bottomrule
% \end{tabular}
% }
% \centering\resizebox{0.43\textwidth}{!}{
% \begin{tabular}{llll|l}
% \toprule
% Places365 & Food101 & Oxford Pets & DTD & \textbf{Avg} \\
% \hline
% 37.36 & 81.26 & 79.97 & 40.80 & 55.90 \\
% 38.71 & 82.32 & 84.36 & 43.03 & 56.84 \\
% \bottomrule
% \end{tabular}
% }
% \caption{Comparison between CLIP with and without the $\texttt{"A photo of a "}$ prompt.}
% \label{tab:prompt}
% \end{table}
\begin{table}[t]
\centering\resizebox{0.34\textwidth}{!}{
\begin{tabular}{l|lll|l}
\toprule
Method & ImageNet & ... & DTD & \textbf{Avg} \\
\hline
CLIP w/o  & 51.87 & ... & 40.80 & 55.90 \\
CLIP + P  & 54.61 & ... & 43.03 & 56.84 \\
\bottomrule
\end{tabular}
}
\caption{Comparison between CLIP with (\textit{+ P}) and without the $\texttt{"A photo of a "}$ prompt. \jm{put this table in Appendix?}}
\label{tab:prompt}
\end{table}

==> tables/interpolation.tex <==
\begin{table}[t]
\centering\resizebox{0.48\textwidth}{!}{
\begin{tabular}{l|l|l|l|l|}
\toprule
Method & ImageNet \cite{?} & EuroSAT \cite{?} & Food101 \cite{?} & Oxford Pets \cite{?} \\
\hline
RCDCLIP  & & & & \\
RCDCLIP with interpolation  & & & & \\
\bottomrule
\end{tabular}
}
\caption{We investigate whether the standard deviation of random character prompt embeddings around a respective center of mass is a suitable confidence measure that can be used to select between original CLIP and the augmented variant.}
\label{tab:interpolation}
\end{table}

==> tables/max_dclip.tex <==
\begin{table}[t]
\centering\resizebox{0.49\textwidth}{!}{
\begin{tabular}{l|lllll}
\toprule
\textbf{ViT-B/32} & ImageNetV2 & ImageNet & CUB200 & EuroSAT & Places365\\
\hline
CLIP~\cite{clip} & 54.71 & 62.01 & 51.28 & 40.78 & 39.12 \\
\hline
DCLIP~\cite{dclip} (\textit{mean})&  \textbf{55.82} & \textbf{63.12} & \textbf{52.47} & \textbf{43.29} & \textbf{40.47}\\
DCLIP~\cite{dclip} (\textit{max})&  54.41   & 61.67   & 52.40   & 37.11   & 37.21\\
\bottomrule
\end{tabular}
}
\centering\resizebox{0.49\textwidth}{!}{
\begin{tabular}{llllll|l}
\toprule
Food101 & Oxford Pets & DTD & Flowers102 & FGVCAircraft & Stanford Cars & \textbf{Avg}\\
\hline
82.59 & 85.06 & 43.18 & 62.89 & 24.99 & 58.54 & 55.01 \\
\hline
\textbf{82.79} & 86.54 & \textbf{43.99} & \textbf{64.01} & \textbf{26.94} & \textbf{57.08} & \blue{\textbf{56.05}} \\
82.37   & \textbf{88.03}   & 43.35   & 63.62   & 25.77   & 56.21   & 54.74  \\
\bottomrule
\end{tabular}
}
\caption{\textbf{Further investigating the importance of description averaging in DCLIP.} We compare the performance of DCLIP where each similarity-score associated with an input image is averaged (\textit{mean}) or where the maximum entry is taken (\textit{max}). As can be seen, averaging makes a significant difference in performance (even underperforming CLIP on average), further highlighting the importance of descriptions averaging compared to the introduction of additional semantics via external LLMs.}
\label{tab:max_dclip}
\end{table}

==> tables/prompt_ensemble.tex <==
\begin{table}[t]
\centering\resizebox{0.49\textwidth}{!}{
\begin{tabular}{l|lllll}
\toprule
\textbf{ViT-B/32} & IN1k-V2 & IN1k & CUB200 & EuroSAT & Places365\\
\hline
CLIP~\cite{clip} & 54.71 & 62.01 & 51.28 & 40.78 & 39.12\\
DCLIP~\cite{dclip} & 55.82 & 63.12 & 52.47 & 43.29 & 40.47\\
\hline
Prompt Ensemble & 55.49 \small$\pm0.21$ & 62.79 \small$\pm0.29$ & 51.46 \small$\pm0.43$ & 45.76 \small$\pm0.49$ & 40.58 \small$\pm0.06$\\
\hline
\ourmodel (ours) & \textbf{55.92} \small$\pm0.08$ & \textbf{63.31} \small$\pm0.09$ & 52.38 \small$\pm0.12$ & 44.31 \small$\pm1.07$ & 40.56 \small$\pm0.07$\\
+ Concepts & $\downarrow$ & $\downarrow$ & \textbf{52.83} \small$\pm0.19$ & \textbf{48.51} \small$\pm0.70$ & \textbf{40.97} \small$\pm0.08$\\
\bottomrule
\end{tabular}
}
\centering\resizebox{0.49\textwidth}{!}{
\begin{tabular}{llllll|l}
\toprule
Food101 & Oxford Pets & DTD & Flowers102 & FGVCAircraft & Cars & \textbf{Avg}\\
\hline
82.59 & 85.06 & 43.18 & 62.89 & 24.99 & 58.54 & 55.01\\
82.79 & 86.54 & \textbf{43.99} & 64.01 & 26.94 & 57.08 & 56.05 \\
\hline
82.67 \small$\pm0.37$ & 83.26 \small$\pm0.72$ & 42.53 \small$\pm0.54$ & 63.30 \small$\pm0.33$ & 25.14 \small$\pm0.45$ & 58.38 \small$\pm0.29$ & 55.58 \small$\pm0.42$\\
\hline
83.25 \small$\pm0.21$ & 85.70 \small$\pm0.25$ & 43.16 \small$\pm0.25$ & 66.27 \small$\pm0.26$ & 25.66 \small$\pm0.19$ & 58.91 \small$\pm0.17$ & 56.31 \small$\pm0.37$\\
\textbf{85.21} \small$\pm0.06$ & \textbf{87.52} \small$\pm0.10$ & $\downarrow$ & \textbf{67.19} \small$\pm0.19$ & \textbf{28.44} \small$\pm0.22$ & \textbf{59.70} \small$\pm0.12$ & \blue{\textbf{57.52}} \small$\pm0.26$\\
\bottomrule
\end{tabular}
}

\caption{\textbf{Comparisons between prompt ensembling, \ourmodel and 
 \ourmodel + concepts}. Across all eleven visual classification benchmarks, we find either matching or improved performance of \ourmodel compared to prompt ensembling (improving on eight out of eleven benchmarks), with the increase in average visual classification performance between \ourmodel and prompt ensembling being higher than the increase when moving from standard CLIP to a prompt-ensembled version, \textbf{without} requiring a handcrafted list of prompts.}
\label{tab:prompt_ensembling}
\end{table}

% \begin{table*}[t]
% \centering\resizebox{0.98\textwidth}{!}{
% \begin{tabular}{l|lllllllllll|l}
% \toprule
% \textbf{ViT-B/32} & IN1k-V2 & IN1k & CUB200 & EuroSAT & Places365 & Food101 & Oxford Pets & DTD & Flowers102 & FGVCAircraft & Cars & \textbf{Avg}\\
% \hline
% CLIP~\cite{clip} & 54.71 & 62.01 & 51.28 & 40.78 & 39.12 & 82.59 & 85.06 & 43.18 & 62.89 & 24.99 & 58.54 & X\\
% DCLIP~\cite{dclip} &  55.82 & 63.12 & 52.47 & 43.29 & 40.47 & 82.79 & 86.54 & \textbf{43.99} & 64.01 & 26.94 & 57.08 & X \\
% \hline
% Prompt Ensemble & 55.49 \small$\pm0.21$ & 62.79 \small$\pm0.29$ & 51.46 \small$\pm0.43$ & 45.76 \small$\pm0.49$ & 40.58 \small$\pm0.06$ & 82.67 \small$\pm0.37$ & 83.26 \small$\pm0.72$ & 42.53 \small$\pm0.54$ & 63.30 \small$\pm0.33$ & 25.14 \small$\pm0.45$ & 58.38 \small$\pm0.29$ & X\\
% \hline
% \ourmodel (ours) & \textbf{55.92} \small$\pm0.08$ & \textbf{63.31} \small$\pm0.09$ & \textbf{52.38} \small$\pm0.12$ & 44.31 \small$\pm1.07$ & 40.56 \small$\pm0.07$ & 83.25 \small$\pm0.21$ & 85.70 \small$\pm0.25$ & 43.16 \small$\pm0.25$ & 66.27 \small$\pm0.26$ & 25.66 \small$\pm0.19$ & 58.91 \small$\pm0.17$ & X\\
% + Concepts & $\downarrow$ & $\downarrow$ & 52.83 \small$\pm0.19$ & 48.51 \small$\pm0.70$ & 40.97 \small$\pm0.08$ & \textbf{85.21} \small$\pm0.06$ & 87.52 \small$\pm0.10$ & $\downarrow$ & 67.19 \small$\pm0.19$ & 28.44 \small$\pm0.22$ & 59.70 \small$\pm0.12$ & X\\
% \bottomrule
% \end{tabular}
% }

% \centering\resizebox{0.98\textwidth}{!}{
% \begin{tabular}{l|lllllllllll|l}
% \toprule
% \textbf{ViT-L/14} & IN1k-V2 & IN1k & CUB200 & EuroSAT & Places365 & Food101 & Oxford Pets & DTD & Flowers102 & FGVCAircraft & Cars & \textbf{Avg}\\
% \hline
% CLIP~\cite{clip} & 67.90 & 73.37 & 62.24 & 56.03 & 40.46 & 92.55 & 93.30 & 52.87 & 74.73 & 44.88 & 76.42 & X\\
% \hline
% DCLIP~\cite{dclip} & \textbf{69.72} & 75.26 & 63.53 & 58.72 & 42.60 & 92.81 & 93.89 & \textbf{56.60} & 78.16 & 51.04 & 75.13 & X\\
% \hline
% Prompt Ensemble & 69.45 \small$\pm0.14$ & 75.13 \small$\pm0.12$ & 63.34 \small$\pm0.24$ & 50.92 \small$\pm0.57$ & 42.00 \small$\pm0.17$ & 93.03 \small$\pm0.17$ & 92.10 \small$\pm0.37$ & 53.90 \small$\pm0.43$ & 74.01 \small$\pm0.53$ & 48.20 \small$\pm0.76$ & 76.68 \small$\pm0.12$ & X\\
% \hline
% \ourmodel (ours) & 69.48 \small$\pm0.08$ & 75.30 \small$\pm0.04$ & \textbf{64.18} \small$\pm0.13$ & \textbf{61.17} \small$\pm0.35$ & 42.26 \small$\pm0.10$ & 93.31 \small$\pm0.09$ & 91.98 \small$\pm0.11$ & 53.94 \small$\pm0.29$ & 76.17 \small$\pm0.27$ & 48.72 \small$\pm0.40$ & 76.71 \small$\pm0.12$ & X\\
% + Concepts & $\downarrow$ & $\downarrow$ & 63.40 \small$\pm0.17$ & 60.20 \small$\pm0.87$ & 42.57 \small$\pm0.09$ & \textbf{93.65} \small$\pm0.05$ & \textbf{94.38} \small$\pm0.08$ & $\downarrow$ & 78.12 \small$\pm0.18$ & 49.45 \small$\pm0.10$ & 76.71 \small$\pm0.14$ & X\\
% \bottomrule
% \end{tabular}
% }

% \centering\resizebox{0.98\textwidth}{!}{
% \begin{tabular}{l|lllllllllll|l}
% \toprule
% \textbf{ResNet50} & IN1k-V2 & IN1k & CUB200 & EuroSAT & Places365 & Food101 & Oxford Pets & DTD & Flowers102 & FGVCAircraft & Cars & \textbf{Avg}\\
% \hline
% CLIP~\cite{clip} & 51.34 & 58.16 & 45.20 & 28.09 & 36.63 & 78.37 & 83.76 & 38.51 & 61.36 & 21.15 & 54.05 & X\\
% \hline
% DCLIP~\cite{dclip} &  \textbf{52.70} & 59.66 & 47.76 & 34.27 & 38.39 & 78.59 & \textbf{85.77} & \textbf{41.01} & 64.86 & 24.48 & 52.59 & X\\
% \hline
% Prompt Ensemble & 52.44 \small$\pm0.23$ & 59.52 \small$\pm0.25$ & 46.60 \small$\pm0.28$ & 36.14 \small$\pm1.08$ & 38.13 \small$\pm0.11$ & 78.51 \small$\pm0.32$ & 82.40 \small$\pm0.59$ & 40.07 \small$\pm0.41$ & 60.99 \small$\pm0.59$ & 22.58 \small$\pm0.17$ & 53.33 \small$\pm0.48$ & X\\
% \hline
% \ourmodel (ours) & \textbf{52.89} \small$\pm0.15$ & \textbf{60.12} \small$\pm0.12$ & 47.68 \small$\pm0.15$ & 31.34 \small$\pm0.47$ & 38.32 \small$\pm0.10$ & 79.68 \small$\pm0.17$ & 84.32 \small$\pm0.20$ & 39.25 \small$\pm0.27$ & 65.25 \small$\pm0.34$ & 23.66 \small$\pm0.04$ & 53.77 \small$\pm0.23$ & X\\
% + Concepts & $\downarrow$ & $\downarrow$ & \textbf{48.34} \small$\pm0.13$ & 35.08 \small$\pm0.42$ & 39.03 \small$\pm0.08$ & \textbf{81.38} \small$\pm0.08$ & \textbf{85.80} \small$\pm0.12$ & $\downarrow$ & 66.58 \small$\pm0.20$ & 24.25 \small$\pm0.09$ & 54.11 \small$\pm0.23$ & X\\
% \bottomrule
% \end{tabular}
% }

% \caption{\textbf{Comparisons to prompt ensembling}.}
% \vspace{-10pt}
% \label{tab:prompt_ensembling}
% \end{table*}







\begin{table}[t]
\centering\resizebox{0.49\textwidth}{!}{
\begin{tabular}{l|lllll}
\toprule
\textbf{ViT-B/32} & IN1k-V2 & IN1k & CUB200 & EuroSAT & Places365\\
\hline
Prompt Ensemble & 55.49 \small$\pm0.21$ & 62.79 \small$\pm0.29$ & 51.46 \small$\pm0.43$ & 45.76 \small$\pm0.49$ & 40.58\\
+ Concepts & $\downarrow$ & $\downarrow$ & \textbf{52.08} \small$\pm0.17$ & \textbf{49.80} \small$\pm0.66$ & \textbf{40.61} \small$\pm0.14$\\
\bottomrule
\end{tabular}
}
\centering\resizebox{0.49\textwidth}{!}{
\begin{tabular}{llllll|l}
\toprule
Food101 & Oxford Pets & DTD & Flowers102 & FGVCAircraft & Cars & \textbf{Avg}\\
\hline
82.67 \small$\pm0.37$ & 83.26 \small$\pm0.72$ & 42.53 \small$\pm0.54$ & 63.30 \small$\pm0.33$ & 25.14 \small$\pm0.45$ & 58.38 \small$\pm0.29$ & 55.58 \small$\pm0.42$\\
\textbf{84.45} \small$\pm0.15$ & \textbf{87.42} \small$\pm0.20$ & $\downarrow$ & \textbf{65.38} \small$\pm0.27$ & \textbf{26.64} \small$\pm0.50$ & \textbf{59.12} \small$\pm0.14$ & \blue{\textbf{56.94}} \small$\pm0.34$\\
\bottomrule
\end{tabular}
}

\caption{\textbf{Prompt ensembling with high-level guidance}. Exactly as with \ourmodel, we apply high-level concept-guidance to prompt ensembling, finding similarly high and consistent improvements in visual classification performance.}
\vspace{-10pt}
\label{tab:prompt_ensembling_concept}
\end{table}

==> tables/random.tex <==
\begin{table}[t]
\centering\resizebox{0.48\textwidth}{!}{
\begin{tabular}{l|l|l|l|l|}
\toprule
Method & ImageNet \cite{?} & EuroSAT \cite{?} & Food101 \cite{?} & Oxford Pets \cite{?} \\
\hline
$l_w = 1, n_w = 1$  & & & & \\
$l_w = 3, n_w = 3$  & & & & \\
$l_w = 5, n_w = 5$  & & & & \\
$l_w = 1, n_w = 5$  & & & & \\
$l_w = 5, n_w = 1$  & & & & \\
\bottomrule
\end{tabular}
}
\caption{Comparison between CLIP, descriptor-based CLIP (DCLIP, \cite{dclip}) and DCLIP with randomly assigned descriptors (RanDCLIP). Note that unlike \cite{dclip}, we utilize the $\texttt{"A photo of a "}$ prompt in all cases.}
\label{tab:random}
\end{table}

==> tables/supp_motivation.tex <==
\begin{table*}[t]
\centering\resizebox{0.98\textwidth}{!}{
\begin{tabular}{l|llllllll|l}
\toprule
\textbf{ViT-B/32} & ImageNetV2 & ImageNet & CUB200 & EuroSAT & Places365 & Food101 & Oxford Pets & DTD & \textbf{Avg}\\
\hline
CLIP~\cite{clip} &  54.71 & 62.01 & 51.28 & 40.78 & 39.12 & 82.59 & 85.06 & 43.18 & 57.34 \\
DCLIP~\cite{dclip} &  \textbf{55.82} & \textbf{63.12} & 52.47 & \textbf{43.29} & 40.47 & 82.79 & 86.54 & \textbf{43.99} & \blue{\textbf{58.56}}\\
\hline
DCLIP (same, 1x)  & 55.47 \small$\pm0.24$ & 62.89 \small$\pm0.19$ & 52.64 \small$\pm0.28$ & 39.74 \small$\pm2.69$ & 40.29 \small$\pm0.47$ & 83.82 \small$\pm0.48$ & 87.04 \small$\pm0.27$ & 43.35 \small$\pm0.41$ & 58.16 \small$\pm1.01$\\
DCLIP (same, 2x) & 55.75 \small$\pm0.21$ & 63.10 \small$\pm0.19$ & \textbf{52.72} \small$\pm0.23$ & 39.73 \small$\pm1.66$ & \textbf{40.61} \small$\pm0.22$ & \textbf{84.01} \small$\pm0.23$ & \textbf{87.10} \small$\pm0.14$ & 43.29 \small$\pm0.22$ & 58.29 \small$\pm0.62$\\
\bottomrule
\end{tabular}
}
\centering\resizebox{0.98\textwidth}{!}{
\begin{tabular}{l|llllllll|l}
\toprule
\textbf{ResNet50} & ImageNetV2 & ImageNet & CUB200 & EuroSAT & Places365 & Food101 & Oxford Pets & DTD & \textbf{Avg}\\
\hline
CLIP~\cite{clip} &  51.34 & 58.16 & 45.20 & 28.09 & 36.63 & 78.37 & 83.76 & 38.51 & 52.51\\
DCLIP~\cite{dclip} &  52.70 & 59.66 & \textbf{47.76} & 34.27 & 38.39 & 78.59 & \textbf{85.77} & \textbf{41.01} & 54.77\\
\hline
DCLIP (same, 1x) & 52.63 \small$\pm0.28$ & 59.69 \small$\pm0.30$ & \textbf{47.76} \small$\pm0.39$ & 32.74 \small$\pm1.49$ & 38.63 \small$\pm0.22$ & 80.08 \small$\pm0.58$ & 85.36 \small$\pm0.52$ & 40.77 \small$\pm0.63$ & 54.71 \small$\pm0.67$\\
DCLIP (same, 1x) & \textbf{52.89} \small$\pm0.23$ & \textbf{59.90} \small$\pm0.26$ & 47.70 \small$\pm0.29$ & \textbf{34.37} \small$\pm1.27$ & \textbf{38.93} \small$\pm0.21$ & \textbf{80.11} \small$\pm0.30$ & 85.34 \small$\pm0.29$ & 40.91 \small$\pm0.79$ & \blue{\textbf{55.02}} \small$\pm0.58$\\
\bottomrule
\end{tabular}
}
\caption{\textbf{Motivating random class descriptors.} Comparing CLIP~\cite{clip} and GPT-descriptor-extended CLIP~\cite{dclip} (DCLIP) with the same set of randomly sampled descriptors used for each class, where the set size is either the average number of descriptions per class in DCLIP (\textit{same, 1x}), or twice that (\textit{same, 2x}). 
%Note that unlike \cite{dclip}, we utilize the \texttt{"A photo of a \{c\}."} prompt in all cases for a fair comparison. 
A random set of descriptors per class can match or even outperform DCLIP 
% the class-specific GPT-3 generated descriptor extension (e.g.\ \texttt{"A photo of a [waffle], which is [a round shape]."}) 
across backbone architectures confirming that randomized prompt averaging leads to higher performance.}
\label{tab:motivation}
\end{table*}

==> tables/used_concepts.tex <==
\begin{table}[t]
\centering\resizebox{0.48\textwidth}{!}{
\begin{tabular}{l|lllll|l}
\toprule
Method & CUB200 & EuroSAT & Places365 & Food101 & Oxford Pets & \textbf{Avg} \\
\hline
CLIP  & & & & & &\\
DCLIP  & & & & & &\\
GPT-X CLIP & & & & & & \\
\bottomrule
\end{tabular}
}
\caption{Using high-level LLM generated concepts (denotes as \textbf{GPT-}e\textbf{X}panded \textbf{CLIP} reveals notable performance improvements over CLIP without having to rely on the use of a dictionary of multiple finegrained descriptors as in DCLIP.}
\label{tab:used_concepts}
\end{table}
